Study of blazars detected by Fermi-LAT as high-energy neutrino sources

Besides the neutrino source detected by IceCube, NGC 1068, the association of the IceCube-170922A neutrino with the blazar in a flaring state among several wavelengths (from radio up to high-energy (HE) gamma-rays), the site and mechanisms of production of HE neutrino remains in discussion. Extragalactic sources such as Quasars, Blazars, Radio galaxies, and Gamma-ray bursts have been proposed as progenitors of HE neutrinos. In this work, we study the Blazars reported by Fermi-LAT in the 4LAC catalog, which are embedded inside the 90\% error of the best-fit position from the neutrinos reported by IceCube. We propose a one-zone lepto-hadronic scenario to describe the broadband Spectral Energy Distribution and then estimate the number of neutrinos to compare with those in the direction of each source. A brief discussion is provided of the results.

==> ChangeLog <==

2023.02.13	v1	first version.   
2023.04.25	v2	fix "skelecton.tex" to use "\onbehalf{..}" for collaboration. 
2023.06.13	v3	fix typo in "PoStemplate_coll.odt".

